Manipulating a Continuous Instrumental Variable in an Observational Study of Premature Babies: Algorithm, Partial Identification Bounds, and Inference under Randomization and Biased Randomization Assumptions

Regionalization of intensive care for premature babies refers to a triage system of mothers with high-risk pregnancies to hospitals of varied capabilities based on risks faced by infants. Due to the limited capacity of high-level hospitals, which are equipped with advanced expertise to provide critical care, understanding the effect of delivering premature babies at such hospitals on infant mortality for different subgroups of high-risk mothers could facilitate the design of an efficient perinatal regionalization system. Towards answering this question, Baiocchi et al. (2010) proposed to strengthen an excess-travel-time-based, continuous instrumental variable (IV) in an IV-based, matched-pair design by switching focus to a smaller cohort amenable to being paired with a larger separation in the IV dose. Three elements changed with the strengthened IV: the study cohort, compliance rate and latent complier subgroup. Here, we introduce a non-bipartite, template matching algorithm that embeds data into a target, pair-randomized encouragement trial which maintains fidelity to the original study cohort while strengthening the IV. We then study randomization-based and IV-dependent, biased-randomization-based inference of partial identification bounds for the sample average treatment effect (SATE) in an IV-based matched pair design, which deviates from the usual effect ratio estimand in that the SATE is agnostic to the IV and who is matched to whom, although a strengthened IV design could narrow the partial identification bounds. Based on our proposed strengthened-IV design, we found that delivering at a high-level NICU reduced preterm babies' mortality rate compared to a low-level NICU for $81,766 \times 2 = 163,532$ mothers and their preterm babies and the effect appeared to be minimal among non-black, low-risk mothers.

==> old_stuff.tex <==

\begin{table}[!ht]
\centering
\caption{Magnitude of encouragement, level of NICU,  mortality and composite outcome in two matched comparisons. (-St-diff- = absolute standardized difference. 1/0 means 1 = yes, 0 = no.)}
\label{tb: comparison}
\scalebox{0.85}{
\begin{tabular}{clccccc} \toprule
 & & \multicolumn{3}{c}{Match 1} & \multicolumn{1}{c}{}
\\ 
\cmidrule(lr){3-5} \cmidrule(lr){6-7} 
 & & Near mean  & Far mean  & -St-diff- &  \\ 
\midrule
Age 35+& Excess travel time to high-level NICU (minutes) & 4.17 & 21.24 & 1.30 &  \\
 &Low-level NICU (1/0) & 0.27 & 0.55 & 0.58 &  \\
 &Dead (1/0) & 0.0159 & 0.0159 & 0 &  \\
  &Composite outcome  & 8.06 & 7.92 & 0.01 &  \\
\bottomrule
\end{tabular}
}
\end{table}

%%% UPDATED 3/5
\begin{table}[!ht]
\centering
\caption{Updated 3/5: Magnitude of encouragement, level of NICU,  mortality and composite outcome in two matched comparisons. (-St-diff- = absolute standardized difference. 1/0 means 1 = yes, 0 = no.)}
\label{tb: comparison}
\scalebox{0.85}{
\begin{tabular}{clccccc} \toprule
 & & \multicolumn{3}{c}{Match 1} & \multicolumn{1}{c}{}
\\ 
\cmidrule(lr){3-5} \cmidrule(lr){6-7} 
 & & Near mean  & Far mean  & -St-diff- &  \\ 
\midrule
Age 35+& Excess travel time to high-level NICU (minutes) & 4.14 & 21.25 & 1.31 &  \\
 &High-level NICU (1/0) & 0.72 & 0.45 & 0.56 &  \\
 &Death (1/0) & 0.0131 & 0.0106 & 0.0223 &  \\
 &Death fetal (1/0) & 0.0039 & 0.0060 & 0.0302 &  \\
 &Death total (1/0) & 0.0170 & 0.0166 & 0.0028 &  \\
 &Length of stay & 7.08 & 7.07 & NA &  \\
  &Composite outcome  & 7.9791 & 7.8791 & 0.0072 &  \\
\bottomrule
\end{tabular}
}
\end{table}

